A Law of Large Numbers for SIR on the Stochastic Block Model: A Proof via Herd Immunity

In this paper, we study the dynamics of the susceptible-infected-recovered (SIR) model on a network with community structure, namely the stochastic block model (SBM). As usual, the SIR model is a stochastic model for an epidemic where infected vertices infect susceptible neighbors at some rate $\eta$ and recover at rate $\gamma$, and the SBM is a random graph model where vertices are partitioned into a finite number of communities. The connection probability between two vertices depends on their community affiliation, here scaled so that the average degrees have a finite limit as the network grows. We prove laws of large numbers (LLN) for the epidemic's trajectory to a system of ordinary differential equations over any time horizon (finite or infinite), including in particular a LLN for the final size of the infection. Our proofs rely on two main ingredients: (i) a new coupling of the SIR epidemic and the randomness of the SBM, revealing a vector-valued random variable that drives the epidemic (related to what is usually called the ``force of the infection'' via a linear transformation), and (ii) a novel technique for analyzing the limiting behavior of the infinite time horizon for the infection, using the fact that once the infection passes the herd immunity threshold it dies out quickly and has a negligible impact on the overall size of the infection.

==> app-notation.tex <==
\section{Summary of Notation}
\label{app:notation}
%\subsection{Model and Notation}
For $n \in \N$ let $G = (V, E)$ be a simple graph on $n$ vertices. 

Graph-based stuff
\begin{itemize}
    \item number of communities K with the set of communities given by $[K]$.
    \item indexing a community - specific community will be $k$ and $\ell$
    \item \khnote{index vertices by $u$ and $v$}
    \item \khnote{overload the $k(\cdot)$ to be the community mapping function}
    \item\cbnote{Use $t$ for continuous time, $\tau$ for stopping times - what should we use for discrete times - I suggest $T$.  We also need a notion for generation times.}
    \item number of vertices in a community - $n_k$
    \item proportion of vertices in a community - $\rho_k = n_k/n$. 
    \item affinity matrix -- $W$ is symmetrix affinity matrix. So $W_{k\ell}$ denotes the probability that there exists and edge between a vertex in community $k$ and community $\ell$. The $1/n$ is \textbf{not} built into the $W$ matrix.
    \item average/degree distribution for a community $D_k = \sum_{\ell \in K} W_{\ell, k} n_{\ell}/n = \sum_{\ell \in K} W_{\ell k} \rho_\ell$
    \item \khnote{in the new notation for Darling, I use $[n_k] = \{v : k(v) = k\}$.}

\end{itemize}

epidemic stuff
\begin{itemize}
    \item $\irt , \rrt$ infection rate and recovery rate 
    \item initial number of infected,susceptible, recovered $S_k(0), I_k(0), R_k(0)$ thus $S_k(t)$ e.t.c denotes number of susceptible etc at time $t$
    \item number of S,I,R in community  $S_k(t), I_k(t), R_k(t)$
    \item differential equations (normalized vs unnormalized) normalized will be $s_k(t) = S_k(t)/n, i_k(t) = I_k(t)/n, r_k(t)  = R_k(t)/n$
    \item ``half-edges'' starting from community $k$: $X_k(t)$  (see coupling to define)
    \item $\chi_k(t) = \int_{0}^t x_k(s) ds$
    \item $Z$ for random walk 
    \item $\theta_k$ survival probability 
    \item stopping times $\tau$ 
    \item Universally: let $S(t) = \sum_k S_k(t)$, $I(t) = \sum_k I_k(t)$, $R(t) = \sum_k R_k(t)$, and $X(t) = \sum_k X_k(t)$
    \item Use $\lambda_{\max}(A)$ to denote the largest eigenvalue of a matrix $A$
    \item $\P(\cdot)$ Probability, $\E[\cdot]$ Expectation
    \item for the graph process, we use $S_k^n(t), I_k^n(t), R_k^n(t)$ and suppress the $n$ if it is clear
    \item for the differential equations, we have $\s(t) = (s_1(t), \dots, s_K(t))$ and similarly for $\i(t), \r(t), \x(t)$
    \item for the graph process $\S^n(t) = (S_1(t), \dots, S_K(t))$ and similarly for $\I, \vec R, \X$.
    \item vector concatenation: for vectors $\u \in \R^n, \v \in \R^m$ then $\w = (\u, \v)$ denotes the vector in $\w \in \R^{n + m}$ such that $w_1 = u_1, \ldots, w_n = u_n, w_{n+1} = v_1, \ldots, w_{n+m} = v_m$
    \item one vertex part : $C_{k\ell} = (D_k)^{-1}W_{k\ell}\rho_\ell D_\ell$; \khnote{I'm calling this matrix $C_\rho$}
    \item upper bound tree part: $(C(t))_{\ell k} = \eta/(\eta + \gamma) S_k(t)W_{\ell k}/n$ (\khnote{this is the stochastic $C$, use $\E[C]$ when you want it for the differential equations}
    \item $(\hat C(t))_{\ell k} = \eta/(\eta + \gamma) s_k(t)W_{\ell k}$
    \item $\Rn = \lambda_{\max}(C(0))$
    \item $\Reff(t) = \lambda_{\max}(C(t))$
    \item $\dReff(t) = \lambda_{\max}(\hat C(t)) = \lambda_{\max}(\E[C(t)]) $
    \item use $G$ for generating functions and $\vec Z_m$ for the generation for branching process
    \item use $L$ for the Lipschitz constant
    \item change $\zeta $ to constants and let $\theta$ be survival probability
    \item $\1$ for the identity matrix $\ind{test}$ for indicator functions
    \item label the fixed $\delta$ (i.e. in Darling), and unlabel the variable error deltas, also label any fixed $\eps$
    \item define $O_p$ and fix all $O$ to be $O_p$ where necessary
    \item \khnote{going to start using $u$ and $v$ for vertices }
\end{itemize}


assumptions: all processes are cadlag
% \subsection{Description of the Epidemic Process}
% \label{sec:epidemic}
% The SIR epidemic on the stochastic block model is a continuous time, Markov chain defined by the 


==> app-unused.tex <==
\section{Martingale Inequalities}
\label{app:martingale}
\begin{lemma}
\label{lem:subm-liminf}
    Suppose that $M_t$ is a submartingale that satisfies the following conditions:
    \begin{enumerate}[(i)]
        \item for some functions $a_t$ such that $a_t = O(\sqrt{t})$, 
        \[
            |M_t - M_{t-1}| \leq a_t
        \]
        \item for some $c > 0$,
        \[
            \E[M_t] \geq \E[M_{t-1}]+c.
        \]
    \end{enumerate}
    Then
    \[
        \liminf_{t\to\infty} \frac{M_t}{t} > 0.
    \]
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:subm-liminf}]
    Let $A_t := \{M_t\leq \delta ct\}$ for some $\delta \in (0, 1)$. By Azuma-Hoeffding and letting $\mu_t = \E[M_t]$ we have
    \begin{align*}
        \sum_{t=1}^\infty \P(A_t) &= \sum_{t=1}^\infty \P(M_t \leq \delta ct) \\
        &\leq \sum_{t=1}^\infty \P(M_t - 1 \leq \delta \mu_t -1 ) \\
        &\leq \sum_{t=1}^\infty \exp\left(-\frac{(\delta \mu_t-1)^2}{2\sum_{k=1}^t a_k^2}\right) \\
        &\leq \sum_{t=1}^\infty \exp\left(- \frac{(\delta (ct + 1) - 1)^2}{2\sum_{k=1}^t a_k^2}\right) \\
        &< \infty
    \end{align*}
    due to the condition on the $a_k$. Thus, by the Borel-Cantelli lemma we can conclude that 
    \[
        \liminf_{t\to\infty} \frac{M_t}{t} \geq \delta c > 0
    \]
    with probability $1$.
    % we have that 
    
    % \begin{align*}
    %     P(A_t \text{ i. o.}) &= P(\limsup_t A_t) \\
    %     &= 1-P(\liminf_t A_t^c) \\
    %     &= 1-P(\liminf_t Y_t \geq \delta tc) = 0.
    % \end{align*}
    
\end{proof}

\section{Poisson Properties}
\begin{lemma}
\label{lem:x_bounded}
For any $\delta >0$, there exists $N \in \Z_+$ s.t. for all $n \geq N$, $x_k(t) \in [0, 1+\delta]$ a.s. 
\end{lemma}

\begin{proof}
    Fix $k \in [K]$, first we prove a concentration bound on $\sup\limits_{t} X_k^n(t)$ (i.e. the maximum number of active edges in community $k$ at any time $t$). Let $v \in [n]$ such that $k(v) = k$ and let $d_v \sim \Pois(D_k)$ be the degree of vertex $v$. Notice that for all $t$, the number of active infective edges in community $k$ is stochastically dominated by sum of $n$ $\Pois(D_k)$   $k$. Thus we have that 
    \[
        \sup\limits_{t} X_k^n(t) \preceq \sum_{v \in [n] : k(v) = k} d_v \preceq \Pois(n D_k) := \overline{X_k^n}.
    \]
    Then, using a Chernoff-type bound we have
    \begin{align*}
        P(\overline{X_k^n}\geq (1+\delta) n D_k) &= P\left(e^{\overline{X_k^n}} \geq e^{(1+\delta)n D_k}\right) \\
        &\leq e^{nD_k(e^s-1) - s(1+\delta)nD_k}. 
    \end{align*}
    Optimizing the RHS over $s$ gives $s = \ln(1 + \delta)$, which gives the bound 
    \begin{align*}
        e^{(\delta - (1 + \delta)\ln(1+\delta))nD_k} = e^{-cnD_k}
    \end{align*}
    for some constant $c > 0$ when $\delta > 0$. 

    \noindent Observe that $P(\overline{X_k^n} \geq (1+ \delta) n D_k) = P(\overline{X_k^n}/n D_k \geq 1 + \delta) > P(\sup\limits_t x_k(t) \geq 1+\delta) $ as $x_k(t) = \frac{X_k^n(t)}{nD_k}$.
    Let $A_n$ be the event that $\{x_k(t) \geq 1+ \delta\}$ by the previous part we know that $P(A_n) < e^{-cnD_k}$ and

    \[
    \sum_{n=1}^\infty P(A_n) < \sum_{n=1}^\infty e^{-cnD_k} = \sum_{n=1}^\infty (e^{-cD_k})^n < \infty 
    \]
    Thus by Borel-Cantelli lemma $P\{ A_n \text{ i.o }\} = 0$. Therefore, $\forall \delta > 0$ there exists $N \in \Z_+$ such that for all $n \geq N$, $\sup\limits_t x_k(t) \in [0, 1+\delta]$. 

\end{proof}

\begin{corollary} \label{cor:lipschitz}
The vector field $b(\y)$ is Lipschitz on $\tilde U$. 
\end{corollary}

\begin{proof}
To show that $b$ is Lipschitz on $\tilde U$ it suffices to check that $b$ is coordinate-wise Lipschitz. To see this, let $b_i(\y)$ denote the $i$th component function of $b(\y)$ and let $\y, \y' \in \tilde U$. Notice that if for each $i$
\begin{equation*}
    |b_i(\y) - b_i(\y')| \leq L_i ||\y - \y'||_2,
\end{equation*}
then
\begin{align*}
    ||b(\y) - b(\y')||_2^2 &\leq \sum_{i=1}^{3K}|b_i(\y) - b_i(\y')|^2 \\
    &\leq \sum_{i=1}^{3K} L_i^2||\y- \y'||_2^2 \\
    &=L ||\y - \y'||_2^2
\end{align*}
with Lipschitz constant $L = \sum_{i=1}^{3K} L_i^2$. The Lipschitz-ness of the $b_i$ follows from the fact that $f(x, y) = xy$ is Lispchitz on any closed rectangle 
\end{proof}

\begin{lemma}[A Chernoff Bound for the Maximum of Poissons]
\label{lem:max-poissons}
    Let $X_i \sim \Pois(\lambda)$ be i.i.d. random variables for $i \in [n]$. Then 
    \[
        \P\left(\max_i X_i \leq t\right) \geq (1 - c_1 e^{-t})^n.
    \]
\end{lemma}

\begin{proof}
\cinote{keep track of the vertices themselves and their active degrees at time t then bound those active degrees by independent poissonsthe}
    \begin{align*}
        \P\left(\max_i X_i \leq t\right) &= \P\left(\forall i, X_i \leq t\right) \\
        &= \prod_{i=1}^n (1 - \P(X_i > t))
    \end{align*}
    By a Chernoff bound,
    \begin{align*}
        \P(X_i > t) & \leq e^{-t}e^{\lambda(e-1)}
    \end{align*}
    so continuing from above, for some constant $c_1 = e^{\lambda(e-1)}$ we have 
    \begin{align*}
       \prod_{i=1}^n (1 - \P(X_i > t)) &\geq  \prod_{i=1}^n(1 - c_1 e^{-t}) = (1 - c_1 e^{-t})^n
    \end{align*}
    Letting $t := (1+\delta)\log n$ for some $\delta \in (0, 1)$ gives 
    \[
        \P\left(\max_i X_i \leq (1+\delta)\log n\right) \geq (1-c_1e^{-(1+\delta)\log n})^n \xrightarrow{n\to\infty} 1. 
    \]
    Where the limit comes from applying l'hopitals rule. This implies that with high probability, $\max_i X_i$ is $O(\log n)$.
\end{proof}

\begin{lemma}[Rate of Convergence for Poissons]
\label{lem:rate-convergence-of-poissons}
Consider the setting as in Theorem \ref{thm:lln}. Then,
\[  
    \P(\norm{\X(0)\cdot \D^{-1}/n - \I(0)/n} \geq \delta/2) = O(1/\delta^2n).
\]
\end{lemma}
\begin{proof}
    We have that 
    \begin{align*}
        \P\left(\left|\frac{\X(0) \cdot \D^{-1}}{n} - \frac{\I(0)}{n}\right| \geq \delta/2\right) &= \P\left(\frac{1}{n}\sum_{k=1}^K |X_k(0)/D_k - I_k(0)| \geq \delta/2\right) \\
        &\leq \sum_{k=1}^K \P\left(\left|\frac{X_k(0)}{D_k} - I_k(0)\right| \geq n\delta/2\right) \\
        &= \sum_{k=1}^K \P\left(\left(\frac{X_k(0)}{D_k} - I_k(0)\right)^2 \geq n\delta/2\right) \\
        &\leq \sum_{k=1}^K \frac{4I_k(0)}{D_k n^2\delta^2} \\
        &\leq \frac{4K I(0)}{\min_k D_k n^2\delta^2}.
    \end{align*}
    In the setting of Theorem \ref{thm:lln}, $I(0) = O(n)$ with probability tending to $1$, thus the overall rate of convergence is $O(1/n)$.
\end{proof}

\begin{lemma}
    Let $X_k$ be as defined in the proof of Theorems \ref{thm:lln} and \ref{thm:LLN} for $k \in [K]$. Then,
    \[
        \P\left(\sum_{k \in [K]} \frac{X_k}{n D_k} \geq 2\right) \leq e^{(1- 2\ln 2)D_0}
    \]
    where $D_0 = \min_k D_k$.
\end{lemma}
\begin{proof}
    Observe that $X_k(t) \preceq \Pois(n_k D_k) \preceq \wt X_k \sim \Pois(nD_k) $, where the first inequality is true since at most $n_k$ vertices can draw a $\Pois(D_k)$ degree. For any random variable $Y \sim \Pois(\lambda)$, by optimizing a Chernoff bound we have 
    \[
        \P(Y \geq 2\lambda) \leq e^{(1-2 \ln 2)\lambda}.
    \]
    Thus, we have 
    \begin{align*}
        \P\left(\sum_{k \in [K]} \frac{X_k}{n D_k} \geq 2\right) &\leq \sum_{k \in [K]} \P\left(\wt X_k \geq 2nD_k\right) \\
        &\leq Ke^{(1-2\ln 2)nD_0} = O(e^{-n}).
    \end{align*}
\end{proof}





==> sec-1-main-results-summary.tex <==
In this paper, we consider an SIR model on a sparse network with community structure, namely the stochastic block model (SBM) with $K$ communities.  The model is defined by dividing the set of nodes into $K$ subsets (communities)  of sizes $n_1,\dots, n_K$ and then connecting each pair of vertices independently at random, with the probability of a connection between vertices of community labels $k$ and $\ell$ being equal to $\frac 1n W_{k\ell}$ where $W$ is a $K\times K$ symmetric matrix with non-negative entries\footnote{We  assume $n$ is chosen large enough to ensure that $\frac 1n W_{k\ell}\leq 1$ for all pairs of labels.}.  
%It is usually assumed  that $n_k/n$ converges to some non-zero density $\rho_k$ as $n\to\infty$.


 
 
We study the SIR epidemic on the stochastic block model. 
We use $k(i)$ for the community label of vertex $i$,  $\mathbf V$ for the set of vertices with their community labels, $\mathbf V=(V,k(\cdot))$, and the notation $G \sim \sbm(\n, W)$ for a graph $G$ drawn from a stochastic block model with affinity matrix $W$.  As usual, the SIR epidemic on $G$ is the continuous time Markov chain defined by the following updates: given the set of susceptible, infected and recovered vertices at time $t$, all infected vertices independently recover at rate $\rrt$, and independently of this, and independently for all edges, each edge between an infected and susceptible vertex transmits the infection at rate $\irt$, with a transmission leading to the susceptible vertex becoming infected.  



To formulate our results, it will be convenient to allow all edges emanating from infected vertices to transmit infections, whether or not the other endpoint is susceptible.  More precisely, it will be convenient to define a set of active edges, by declaring all edges coming out of a vertex to be active when a vertex initially gets infected.  Once active, edges will transmit infections at rate $\irt$.  The first time such a transmission happens, the other endpoint, if susceptible, becomes infected, and otherwise does not change its state.  Furthermore, the edge becomes inactive.  Clearly, this extension does not change the dynamics of the set of susceptible, infected, and recovered vertices.


To formulate our first result, the law of large number for the infection, we use $S_k(t)$, $I_k(t)$ and $R_k(t)$ to denote the number of  susceptible, infected, and recovered vertices in community $k$, respectively.  We also introduce the 
\emph{force  of the infection emanating from vertices of label $k$}, defined as the number $X_k$ of active edges emanating from vertices of community label $k$.  As we will see, it is the force of the infection, rather than the number of currently infected vertices which drives new infections, and hence the dynamic of the infection. 

Let $D_{k}=\sum_{\ell}W_{k\ell} n_\ell/n$. 

% \khnote{I just realized that we never define $\rho_\ell$ before we use it.}
% \cbnote{I think we can use $n_k/n$, which has been defined}
Our first theorem states that the normalized quantities $S_k(t)/n$, $I_k(t)/n$
and $X_k(t)/(n D_k)$ converge to the solution of the following differential equations.

\begin{align}
\label{eq:s_dfq'}
    \frac{d}{dt}s_k(t) &= -\irt  \sum_\ell x_\ell(t) W_{ \ell k}s_k(t);
    \\
\label{eq:x_dfq'}
    \frac{d}{dt}x_k(t) &= -  \frac{d}{dt}s_k(t)
    -(\irt + \rrt) x_k(t);
\\
\label{eq:i_dfq'}
    \frac{d}{dt}i_k(t) &=  -  \frac{d}{dt}s_k(t)
    -\rrt i_k(t);
    \\
\label{eq:r_dfq'}
   r_k(t) &= \rho_k-s_k(t)-i_k(t).
\end{align}

Before stating our precise results, let us motivate these equations.  To this end, we observe that  the probability that a vertex in community $\ell$ points to a given vertex in community $k$ is $\frac 1nW_{\ell k}$. On average, an edge pointing out of a vertex in community $\ell$ thus has probability $\frac 1{n D_\ell} W_{\ell k}$ of pointing to a given vertex in community $\ell$.  Thus the rate at which
susceptible vertices get infected is asymptotically equal to
$$
\irt \sum_\ell  \frac {X_\ell}{nD_{\ell}}W_{\ell k} S_k,
$$
leading to the first equation.  The second follows by observing that on average, a newly infected vertex of label $k$ creates $D_k$ new active edges, which on average leads to a change of $+1$ in $X_k/D_k$. Combined with the fact that active edges disappear either when the infected endpoint recovers or the edge transmits an infection, this leads to the second equation.  The third equation follows from the fact that a successful infection event moves exactly one vertex from susceptible to infected (explaining the first term), and that a recovering event removes precisely one infected vertex.  The last equation is just the fact that the infection does not change community labels.




\begin{theorem} Consider an SIR-dynamic on a graph 
$G \sim \sbm(\n, W)$, with the initial sets of infected and recovered vertices chosen uniformly without replacement in each community, with the number of infected and recovered vertices chosen in such a way that
$S_k(0)/n=(n_k-I_k(0)-R_k(0))/n$, $I_k(0)/n$, and $R_k(0)/n$ converge to some (not necessarily non-zero) numbers $s_k(0)$, $i_k(0)$ and $r_k(0)$. 
Fix some finite time horizon $0<t_0<\infty$. Then
\begin{align}
\label{s_d-conv}\sup_{t\in [0,t_0]}\left| \frac{S_k(t)}n-s_k(t)\right|&\pto 0;
    \\
\label{x_d-conv}
    \sup_{t\in [0,t_0]}\left| \frac{X_k(t)}{nD_k}-x_k(t)\right|&\pto 0;
\\
\label{i_d-conv'}
   \sup_{t\in [0,t_0]}\left| \frac{I_k(t)}n-i_k(t)\right|&\pto 0;
    \\
\label{r_df-conv}
    \sup_{t\in [0,t_0]}\left| \frac{R_k(t)}n-r_k(t)\right|&\pto 0
\end{align}
where the convergence is in probability with respect to both the randomness of $G$ and that of the SIR dynamic, and $s_k(t)$, $x_k(t)$, $i_k(t)$ and $r_k(t)$ are the unique solutions to \eqref{eq:s_dfq'} --
\eqref{eq:r_dfq'} with initial conditions  $s_k(0)$, $i_k(0)$, $r_k(0)$ and $x_k(0)=i_k(0)$.
\end{theorem}

While the heuristic ideas leading to the statements of the theorem are intuitive, the actual proof requires a careful analysis of the interplay of the randomness of $G$ and that of the infection, which we will do by first coupling the graph $G$ to a certain multi-graph $G'$, and then coupling the dynamic of the infection to the randomness of $G'$.  Once this coupling is established, we will use tools that are standard when proving laws of large numbers, following closely the approach of \cite{darling08:dfq-markov}, which in turn is based on Doob’s inequality and Gronwall’s lemma. 

Gronwall's lemma, stated as in the form used in \cite{darling08:dfq-markov} says that, for any real-valued integrable function $f$ on the interval $[0, t_0]$, the inequality
\[
    f(t) \leq C + D \int_0^t f(s)\, ds \text{ for all }t
\]
implies that $f(t_0) \leq Ce^{Dt_0}$. However, the errors grow exponentially large as $t_0$ tends to infinity, which makes it difficult to analyze the final size of the infection directly. Traditionally, this is solved by using a time change and renormalizing the jump rates as done in \cite{darling08:dfq-markov}\cite{janson14:lln-sir}. In this paper, we introduce a new method of getting around the difficulties of using Gronwall's inequality directly by using properties of the backwards birth process at the end of the infection. 

 % \khnote{sir on complete graph (cite darling), using rescaling you can prove final size (darling), use a new method not rescaling - describe the birth process argument for the SIR model, to show the usefulness of the method apply it to SBM, to our knowledge has not been done, in words explain how to do it for the final size, furthermore we also prove the results starting from the single vertex}







%\subsection{Main Results}
% Using methods from \cite{darling08:dfq-markov}, we will show that for appropriately scaled $S_k(t), I_k(t), R_k(t), X_k(t)$, these processes converge to deterministic functions that solve an ordinary differential equation. Throughout the following sections, let $G^*$ be the multigraph drawn from the half-edge coupling described above. 


% Here, we first introduce some notation to be consistent with the notation in \cite{darling08:dfq-markov}, let $Y = (Y_t)_{t \geq 0}$ denote the SIR epidemic on the stochastic block model with countable state-space $S$ consisting of elements of the form 
% \[
%     \xi = (s_1, \dots, s_K, i_1^0, i_1^1, \dots, i_2^0, \dots, i_K^0, \dots, r_1,\ldots,  r_K).
% \]

% We do not need to include the number of recovered vertices in each community, because this is determined by the number of susceptible and infected vertices in each community. 
% \cinote{this is probably true but we're now drawing the colors from fixed distribution can think about this later but i
% m including the recoverd for now}

% \cbnote{You will also want that $X_k(0)/n$ and all the other relevant quantities converge, see my email from May 10, and you will want to allow for more general starting conditions than Poisson degrees with expectation $D_k$.}
% \begin{restatable*}[Law of Large Numbers]{theorem}{lln}
% \label{thm:lln}
%     Consider the SIR epidemic on $G^*$ where new, infective vertices in community $k$ are given Poisson degrees according to $\Pois(D_k)$. Fix $\eps \in (0, 1)$ suppose that the following initial conditions are satisfied:
%     \begin{enumerate}[(i)]
%         \item the maximum degree of any initially infective vertex is at most $n^{1/2}$
%         \item $\sum_k s_k(0) < 1$.
%     \end{enumerate}
%     Let $s_k(t), i_k(t), r_k(t), x_k(t)$ be the unique solutions to 
%     \begin{equation}\label{s_diff_eq_1}
%         \frac{ds_k}{dt} = -\irt s_k \sum_\ell x_\ell 
%         {W_{\ell, k}}
%     \end{equation}
    
%     \begin{equation}\label{x_diff_eq_1}
%         \frac{dx_k}{dt} = -(\irt + \rrt) x_k + \irt s_k \sum_\ell x_\ell W_{\ell, k}
%     \end{equation}
%     \begin{equation}
%         \frac{di_k}{dt} = -\rrt i_k + \irt s_k \sum_\ell x_\ell 
%         {W_{\ell, k}}
%     \end{equation}
%     \begin{equation}
%         \frac{dr_k}{dt} = \rrt i_k.
%     \end{equation}
%     Then, uniformly on the interval $[0, t_0]$,
%     \[
%         \frac{S_k(t)}{n} \pto s_k(t), \quad \frac{X_k(t)}{nD_k} \pto x_k(t), \quad \frac{I_k(t)}{n} \pto i_k(t), \quad \frac{R_k(t)}{n} \pto r_k(t)
%     \]
%     as $n$ tends to infinity, for any $t_0 > 0$. 
% \end{restatable*}
% The next theorem extends Theorem \ref{thm:lln} to the case where there are very few initially infective vertices. Let $C(t)$ be the matrix with elements $(C(t))_{k\ell} = \irt S_k(t) W_{k \ell}/n$. The following two quantities will be of interest in the analysis:
% \begin{equation}
%     \Rn := \E[\lambda_1(C(0))]
% \end{equation}
% and 
% \begin{equation}
%     \Reff(t) := \E[\lambda_1(C(t))],
% \end{equation}
% where $\lambda_1(\cdot)$ denotes the largest eigenvalue. $\Rn$ can be interpreted as the basic reproductive ratio of the epidemic, and $\Reff(t)$ can be interpreted as the effective reproductive ratio at time $t$ during the course of the epidemic. Fix $\eps \in (0, 1-\max_k s_k(\infty))$ and let
% \khnote{changed it to the total}
% \[
%     \tau_\eps := \inf\{t \geq 0: S(t) \leq n(1-\eps)\}
% \]
% where $s_k(\infty)$ is the (approximate) fraction of susceptible vertices in community $k$ at the end of the epidemic in the event that a large outbreak occurs.

%\onevertex


% \begin{restatable*}{theorem}{onevertex}
% \label{thm:onevertex}
%     Consider the SIR epidemic on $G^*$.
%     % where new, infective vertices in community $k$ are given Poisson degrees according to $\Pois(D_k)$. 
%     Suppose that $\sum_k I_k(0) = O(1)$ but there is at least one infective vertex with nonzero degree. There exists constants $C$ and $\eps_0$ such that for $\eps < \eps_0$ the following holds:
%     \begin{enumerate}[(a)]
%         \item if $\Rn \leq 1$, then $\{\tau_{\eps} = \infty\}$ with high probability and there exists a time $\tau_1$ such that for all $k\in [K]$, $X_k(\tau_1) = 0$,
%         \item if $\Rn > 1$, then $P(\tau_{\eps} < \infty) > 0$  and conditioned on the event that $\{\tau_\eps < \infty\}$, there exists a $k \in [K]$, such that  $X_k(\tau_\eps) > C \eps n$. 
%     \end{enumerate}
%     \khnote{formulate the birth process with matrix $C$. let $p$ be the probability that that one dies out. if $\Rn > 1$, probability -> $p$}
% \end{restatable*}

==> sec-complete-graph-example.tex <==
\subsection{Motivating Example on the Complete Graph}
In this section, we illustrate our new method by analyzing convergence of the final infection size in the SIR infection on the complete graph. Consider all the notation in this section to be self-contained.

Let $K_n$ be a complete graph on $n$ vertices and let $S^n(t), I^n(t), R^n(t)$ denote the numbers of susceptible, infectious, and recovered vertices at time $t$ respectively. Note that we may sometimes remove the dependency on $n$ in the superscript for convenience of notation. We use the setup of \cite{darling08:dfq-markov}. Let $\irt$ correspond be the infection rate and $\rrt$ be the recovery rate. The state space for this Markov Chain is the set $S = \{\xi = (\xi^1, \xi^2, \xi^3) , \xi^1 + \xi^2 + \xi^3 = n, \xi \in \Z_3^+\}$. The non-zero jump rates, for $\xi, \xi' \in S$ are given by
\[
    q(\xi, \xi') = \begin{cases}
        \irt \xi^1\xi^2 / n & \xi' = \xi + (-1, 1, 0) \\
        \rrt \xi^2 & \xi' = \xi + (0, -1, 1).
    \end{cases}
\]

Then, as shown in \cite{darling08:dfq-markov}, we have the following theorem:
\begin{theorem}
\label{thm:lln-complete-graph}
    For any finite $t_0 > 0$, on $[0, t_0]$, 
    \begin{equation}
        \sup_{t\in [0, t_0]} \left | \frac{S(t)}{n} - s(t) \right | \pto 0
    \end{equation}
    \begin{equation}
        \sup_{t \in [0, t_0]} \left | \frac{I(t)}{n} - i(t) \right| \pto 0 
    \end{equation}
    \begin{equation}
        \sup_{t \in [0, t_0]} \left | \frac{R(t)}{n} - r(t) \right| \pto 0.
    \end{equation}
    where $s(t), i(t), r(t)$ are the unique solutions to the following system of differential equations:
    \begin{equation}
        \frac{d}{dt} s(t) = - \irt s(t) i(t)
    \end{equation}
    \begin{equation}
        \frac{d}{dt} i(t) = - \rrt i(t) + \irt s(t) i(t)
    \end{equation}
    \begin{equation}
        \frac{d}{dt} r(t) = \rrt i(t)
    \end{equation}
    with initial conditions $x_0 = (1-\eps, \eps, 0)$ for some $\eps \in (0, 1)$.
\end{theorem}

Darling then proceeds to show that, using a time change and dividing the jump rates by $\wt q(\xi, \xi') = q(\xi, \xi') / \xi^2$, as well as using the explicit solution of the differential equation, we obtain a new process and the following theorem:
\begin{theorem}
\label{thm:final-size-complete}
    Let $\rho$ be the unique root of the equation
    \[
        \rho + (1-\eps) e^{-\lambda \rho} = 1. 
    \]
    Then
    \begin{equation}
        |R(\infty) - \rho| \pto 0.
    \end{equation}
\end{theorem}

The proof of this in \cite{darling08:dfq-markov} heavily relies on the fact that the Lipschitz constant of the vector field for the differential equations remains the same after the time change. However, we will see that there is no simple way to make a similar time change in the case of the SIR epidemic on the stochastic block model. We now prove Theorem \ref{thm:final-size-complete} using our new birth process method.

\subsubsection{Birth Process Method}

\begin{lemma}
\label{lem:diff-eq-lim-complete-graph}
    Starting from initial conditions $(1-\eps, \eps, 0)$, the solutions to the differential equations have a limit as $t \to \infty$ and in particular, $i(t) \to 0$ as $t \to\infty$.
\end{lemma}

\begin{proof}
    Notice that $\frac{d}{dt}s(t)$ and $\frac{d}{dt} r(t)$ are monotonically decreasing and increasing in $t$, respectively. Thus by the monotone convergence theorem, since $s(t)$ and $r(t)$ are bounded above by $1$, $s(t)$ and $r(t)$ have a limit as $t$ goes to infinity. Furthermore, since $s(t) + i(t) + r(t) = 1$ for all $t$ (the overall change in the whole system for any $d t$ is $0$), this implies that $i(t)$ must also converge to a limit as $t$ goes to infinity.

    Using the explicit form for the solution of the differential equations, 
    \[
        r(t) = \gamma \int_0^t i(u) \, du.
    \]
    Since $r(t)$ converges to a limit in $(0, 1)$ and $i(t)$ is non-negative for all $t$, this implies that $i(t) \xrightarrow{t \to\infty} 0$.
\end{proof}

\begin{corollary}
\label{cor:subcritical-complete-graph}
    A corollary of Lemma \ref{lem:diff-eq-lim-complete-graph} is that there exists a time $t_1$ such that $\irt s(t) - \gamma < 1$ for all $t \in [t_1, \infty)$. In particular, this implies that the infection is subcritical after time $t_1$. 
\end{corollary}

\begin{proof}
    This corollary follows from the fact that $i(t)$ converges to $0$ with $t$. This implies that there exists a time $t_1$ such that $i(t)$ is subcritical at $t_1$. Since $s(t)$ decreases monotonically, this implies that 
    \[
        \irt s(t) - \gamma < \irt s(t_1) - \gamma < 1
    \]
    for all $t > t_1$. 
\end{proof}

\begin{theorem}
    With initial conditions $(s(0), i(0), r(0)) = (1-\eps, \eps, 0)$, 
    \[
        \left | R(\infty) - \rho\right| \pto 0.
    \]
\end{theorem}

\begin{proof}
    Notice that, under the initial conditions specified in Lemma \ref{lem:diff-eq-lim-complete-graph}, using the explicit for for the solution to the differential equations, we have that $r(\infty)$ is the unique solution to the equation
    \begin{equation}
        (1-\eps) e^{-\irt / \rrt \cdot r(\infty)} + r(\infty) = 1.
    \end{equation}
    In order to show that the final size of the stochastic epidemic itself converges to $r(\infty)$, we will use the following two facts:
    \begin{fact}
        For all $\delta > 0$, there exists $N, \tau_0$ such that 
        \[
            \frac{R^N(\infty)}{N} \geq r(\infty) - \eps.
        \]
    \end{fact}
    \begin{proof}
        By Theorem \ref{thm:lln-complete-graph}, there exists $N, t_0$ such that for all $n\geq N$,
        \[
            r(\infty) - \eps \leq \frac{R^N(t_0)}{N} \leq \frac{R^N(\infty)}{N}
        \]
        where the last inequality is true since $R^N(t)$ is monotonically increasing in $t$.
    \end{proof}
    \begin{fact}
        For all $\delta > 0$, there exists $N$ such that 
        \[
            \frac{R^N(\infty)}{N} \leq r(\infty) + \eps.
        \]
    \end{fact}
    \begin{proof}
        Notice that 
        \begin{equation}
            \frac{R^N(\infty)}{N} \leq \frac{R^N(\tau_1)}{N} + \frac{I^N(\tau_1)}{N} + \frac{|S^N(\infty) - S^N(\tau_1)|}{N}
        \end{equation}
        where $\tau_1$ is chosen such that the infection is subcritical and such that $\frac{I(\tau_1)}{N} < \eps_1$ for some $\eps_1 > 0$. This can be done due to Theorem \ref{thm:lln-complete-graph} and Corollary \ref{cor:subcritical-complete-graph}. Finally, notice that $|S^N(\infty) - S^N(\tau_1)|$ is the same as the number of vertices that become infected between time $\tau_1$ and $\infty$. Since $\irt s(\tau_1) i(\tau_1) > \irt s(t) i(t)$ for all $t \geq \tau_1$, we can upper bound the number of vertices that become infected after time $\tau_1$ by the size of a subcritical branching process, $\cal B$, with offspring distribution $\Pois(\irt/(\irt + \rrt) S^N(\tau_1))$. 
        
        can be bounded above by the number of infection events that occur from time $\tau_1$ until $\infty$. We will see that this corresponds to a subcritical branching process that has died out and has size $o(N)$. 
    \end{proof}
\end{proof}

==> sec-one-vertex-final-size.tex <==
\begin{theorem}
Starting from arbitrary initial conditions for $x_k(0)$ and $ \sum_k s_k(0) < 1 $ we show that as $t \to \infty$,  $r_k(\infty) \to \rho_k(1 - \zeta_k^\infty)$  where $\zeta_k^\infty $ is the unique  solution to the following equation 
\begin{equation}
    \boxed{\zeta_k^\infty = \frac{s_k(0)}{\rho_k}\exp\left\{-\frac{\irt}{\irt + \rrt}\sum_\ell W_{\ell k}\rho_\ell\left(\frac{x_\ell(0) + s_\ell(0)}{\rho_\ell}-\zeta_\ell^\infty\right) \right\} }
\end{equation}


    
\end{theorem}

\cinote{show that the largest non-zero solution is the one that corresponds to the $\zeta_k^{\infty}$}

\cinote{Use the approximate survival probability for $k$ generations then at least one of my children must survive at least $k-1$ generations. Then use the branching process to get the recurrence and we know that the actual one is the limit and compare that to the solution of this implicit equation and must be bounded above and below and then the lowest solution will be the correct one. there's any other solution then it will be the smallest prove for multitype}
From \eqref{eq:s_dfq} and \eqref{eq:x_dfq} from Section \ref{sec:lln} we get
\begin{equation*}
    \frac{d}{dt}s_k(t) = -\irt s_k(t) \sum_\ell x_\ell(t) W_{\ell, k} \tag{\ref{eq:s_dfq}}
\end{equation*}

\begin{equation*}
    \frac{d}{dt}x_k(t) = -(\irt + \rrt) x_k(t) + \irt s_k(t) \sum_\ell x_\ell(t) W_{\ell, k}  \tag{\ref{eq:x_dfq}}
\end{equation*}


\noindent First, rearrange \eqref{eq:s_dfq} and solve to get 
\begin{align}
    \frac{1}{s_k(t)}\frac{ds_k(t)}{dt} &= - \irt \sum_\ell x_\ell(t) W_{\ell k} \nonumber \\
    \log s_k(t) - \log s_k(0) &= -\irt \sum_\ell W_{\ell k} \int_{0}^t x_\ell(\tau) d\tau \nonumber \\
    s_k(t) &= s_k(0)\exp\left\{-\irt \sum_\ell W_{\ell k}\chi_\ell(t)\right\}. \label{eq:s_0_sol}
\end{align}

Where $\chi_k(t) = \int_{0}^t x_k(\tau) d\tau $
\noindent Rearrange \eqref{eq:x_dfq} for $x_k(t)$ to get 
\begin{align*}
    -(\irt + \rrt) x_k(t) &= \frac{dx_k(t)}{dt} + \frac{ds_k(t)}{dt} \\
    x_k(t) &= -\frac{1}{\irt + \rrt}\left(\frac{dx_k(t)}{dt} + \frac{ds_k(t)}{dt}\right).
\end{align*}

\noindent Thus,

\begin{equation}
    \frac{d\chi_k(t)}{dt} + \frac{1}{\irt + \rrt}\left(\frac{dx_k(t)}{dt} + \frac{ds_k(t)}{dt}\right) = 0
\end{equation}
and
\begin{equation}
\chi_k(t) + \frac{1}{\irt + \rrt}\left(x_k(t) + s_k(t) \right) = \frac{x_k(0) + s_k(0)}{\irt + \rrt}
\end{equation}



where the constant on the rhs above is based on the initial conditions. At time $t = \infty$, $x_k(t) = 0, \forall k \in [K]$ 


\begin{equation}
    \chi_k(\infty) + \frac{1}{\irt + \rrt}s_k(\infty) = \frac{ x_k(0) + s_k(0)}{\irt + \rrt}
\end{equation}
which implies that 
\begin{equation}
    \chi_k(\infty) = \frac{x_k(0) + (s_k(0) - s_k(\infty))}{\irt + \rrt}.
\end{equation}
\begin{align*}
    s_k(\infty) &= s_k(0)\exp\left\{-\irt \sum_\ell W_{\ell k}\chi_\ell(\infty)\right\} \\
    &= s_k(0)\exp\left\{-\irt \sum_\ell W_{\ell k}\frac{x_\ell(0) + (s_\ell(0) - s_\ell(\infty))}{\irt + \rrt}\right\} \\
    &= s_k(0)\exp\left\{-\frac{\irt}{\irt + \rrt}\sum_\ell W_{\ell k}( x_\ell(0) + s_\ell(0) - s_\ell(\infty))\right\}
\end{align*}
\begin{equation}
    s_\ell(\infty) + r_\ell(\infty) = \rho_k
\end{equation}
therefore 

\begin{equation*}
    \rho_k - r_k(\infty) = s_k(0)\exp\left\{-\frac{\irt}{\irt + \rrt}\sum_\ell W_{\ell k}(x_\ell(0) + s_\ell(0) - \rho_k + r_\ell(\infty))\right\}
\end{equation*}


% \begin{equation*}
%     \rho_k - r_k(\infty) = \exp\left\{-\frac{\irt}{\irt + \rrt}\sum_\ell W_{\ell k}(r_\ell(\infty) - \rho_k)\right\}\exp\left\{\frac{(\irt + \rrt)\log(s_k(0)) -\irt}{\irt + \rrt}\sum_\ell W_{\ell k}((\irt + \rrt + 1) x_\ell(0) + s_\ell(0)) \right\}
% \end{equation*}

Let $\zeta_k^\infty = 1 - \frac{r_k(\infty)}{\rho_k}$


\begin{equation}
    \boxed{\zeta_k^\infty = \frac{s_k(0)}{\rho_k}\exp\left\{-\frac{\irt}{\irt + \rrt}\sum_\ell W_{\ell k}\rho_\ell\left(\frac{x_\ell(0) + s_\ell(0)}{\rho_\ell}-\zeta_\ell^\infty\right) \right\} }
\end{equation}


==> sec-pair-approx.tex <==
To confirm the correctness of our model and differential equations, we can heuristically derive another set of differential equations that coincides with those given by the pair approximation. Consider the model from Section \ref{sec:coupling} modified slightly in the following way: only consider active edges that will connect to susceptible individuals. In other words, when a vertex in community $k$ is infected, we give it $\Pois(D_k n^{-1}W_{k\ell}s_\ell)$ active, infective edges to susceptible vertices in community $\ell$. Since we only consider links to susceptible vertices, we also delete any active, infective edges in community $k$ with probability $\left(s_k \sum_\ell W_{\ell k}\right)^{-1}$. Let $x_{k\ell}$ denote the number of active, infective edges from community $k$ into susceptible vertices in community $\ell$. Then, we have the following system of differential equations \khnote{not sure if this is correct...}:
\begin{align}
    \frac{ds_k}{dt} &= - \irt s_k \sum_j x_{jk} \\
    \frac{di_k}{dt} &= - \rrt i_k + \irt s_k \sum_j x_{jk} \\
    \frac{dr_k}{dt} &= \rrt i_k \\
    \frac{dx_{k\ell}}{dt} &= -(\irt + \rrt) x_{k\ell} + \irt \sum_j x_{jk} D_k \frac{W_{k\ell}}{n}s_\ell - \irt \frac{x_{k\ell}^2}{s_k \sum_\ell W_{k\ell}}.
\end{align}




Consider a graph $H$ on $n$ nodes drawn from the coupled process and let $G$ be the adjacency matrix of the graph. The expected adjacency matrix of the graph corresponds with the distribution where $D_\ell^{-1} W_{\ell k} \rho_k$ is the probability that a vertex of type $\ell$ matches to a vertex of type $k$. In particular the $ij$th entry $\E[G]_{ij} = D_{k(i)}^{-1} W_{k(i), k(j)}\rho_{k(j)}$, where $k(i)$ denotes the community of vertex $i$. Let $A \in \{S_1, \dots, S_q, I_1, \dots, I_q, R_1, \dots, R_q\}$ and $i \in [n]$ where $A_i = 1$ if node $i$ is of type $A$ and $A_i = 0$ otherwise. Also, let 
\[
    [A]_n = \sum_{i=1}^n A_i, \quad [AB]_n = \sum_{i, j=1}^n A_i g_{ij} B_j, \quad [ABC]_n = \sum_{\substack{i, j, k = 1 \\ i \neq k}}^n A_i g_{ij} B_j g_{jk} C_k.
\]
Suppose that $n^{-1}[A]_n , n^{-1} [AB]_n, n^{-1}[ABC]_n$ tend to deterministic limits as $n\to\infty$. Denote the limits (for example)
\[
    n^{-1}[S_k]_n \to s_k, \quad n^{-1}[S_k I_\ell] \to x_{s_k i_\ell}.
\]
Then, a heuristic argument yields the following system of deterministic differential equations to describe the system:
\begin{align}
    \frac{ds_k}{dt} &= - \irt \sum_{\ell} x_{s_k i_\ell} \\
    \frac{di_k}{dt} &= - \rrt i_k + \irt \sum_{\ell} x_{s_k i_\ell} \\
    \frac{dx_{s_k i_\ell}}{dt} &= - \rrt x_{i_\ell s_k} - \irt x_{i_\ell s_k} + \irt \sum_j x_{i_j s_\ell s_k} - \irt x_{i_\ell s_k i_\ell} \label{xsi}.
\end{align}
The first term in \ref{xsi} comes from the rate at which $i_\ell$ vertices recover, which removes an $i_\ell s_k$ link. The second term comes from the fact that when a infective vertex infects down an edge to a susceptible, that link goes from an $i_\ell s_k$ to an $i_\ell i_k$ link. The third term comes appears because at rate $\irt$ an infection is sent down an $i_j \to s_\ell$ edge, which then increases the number of $i_\ell i_k$ links. The last terms comes because the rate and intensity of infection are both doubled (when there is an $i_\ell s_k i_\ell$ link and an infection is sent, it is sent at twice the rate and two $i_\ell s_k$ links are deleted). To close the system, we use the pair approximation
\[
    x_{ABC} = \frac{x_{AB}x_{BC}}{x_B}
\]
in equation \ref{xsi}, which gives
\begin{equation}
\label{xsi_approx}
    \frac{dx_{s_k i_\ell}}{dt} = - \rrt x_{s_k i_\ell} - \irt x_{s_k i_\ell} + \irt \sum_{j} \frac{x_{i_j s_\ell}x_{s_\ell s_k}}{s_\ell} - \irt \frac{x_{i_\ell s_k}x_{s_k i_\ell}}{s_k}.
\end{equation}
Notice that 
\begin{equation}
\label{ss}
    x_{s_\ell s_k} = s_k(t) s_\ell(t) \frac{W_{\ell k}}{n}
\end{equation}
is just the expected number of edges between susceptibles in communities $k$ and $\ell$. Plugging \ref{ss} into \ref{xsi_approx} gives
\begin{equation}
\label{xsi_final}
    \frac{dx_{s_k i_\ell}}{dt} = -\rrt x_{s_k i_\ell} - \irt x_{s_k i_\ell} + \irt \sum_j x_{i_j s_\ell} s_\ell\frac{W_{\ell k}}{n} - \irt\frac{x_{i_\ell s_k}^2}{s_k}.
\end{equation}


